Enabling Content Management Systems as an Information Source in Model-driven Projects

Content Management Systems (CMSs) are the most popular tool when it comes to create and publish content across the web. Recently, CMSs have evolved, becoming \emph{headless}. Content served by a \emph{headless CMS} aims to be consumed by other applications and services through REST APIs rather than by human users through a web browser. This evolution has enabled CMSs to become a notorious source of content to be used in a variety of contexts beyond pure web navigation. As such, CMS have become an important component of many information systems. Unfortunately, we still lack the tools to properly discover and manage the information stored in a CMS, often highly customized to the needs of a specific domain. Currently, this is mostly a time-consuming and error-prone manual process. In this paper, we propose a model-based framework to facilitate the integration of headless CMSs in software development processes. Our framework is able to discover and explicitly represent the information schema behind the CMS. This facilitates designing the interaction between the CMS model and other components consuming that information. These interactions are then generated as part of a middleware library that offers platform-agnostic access to the CMS to all the client applications. The complete framework is open-source and available online.

==> utils/collab.tex <==
\RequirePackage{xcolor}
\RequirePackage[normalem]{ulem}
\RequirePackage[textsize=scriptsize,textwidth=3.2cm,color=orange!25,linecolor=orange]{todonotes}
\RequirePackage[scaled]{helvet}

% Enable page numbering
\pagestyle{plain}

% \comment{Comment}
% \comment[author]{Comment}
\newcounter{comment}
\newcommand{\comment}[2][]{%
\refstepcounter{comment}{%
{\renewcommand{\baselinestretch}{1.0}
\todo{\fontfamily{phv}\fontseries{bc}\selectfont%
Comment [#1\thecomment]: %
\fontfamily{phv}\fontseries{mc}\selectfont#2}}}}

% \add{Text to add}
% \add[author]{Text to add}
\newcommand{\add}[2][]{%
\if\relax\detokenize{#1}\relax%
\else\todo{\fontfamily{phv}\fontseries{bc}\selectfont#1}%
\fi%
{\color{teal}#2}}

% \del{Text to delete}
% \del[author]{Text to delete}
\newcommand{\del}[2][]{%
\if\relax\detokenize{#1}\relax%
\else\todo{\fontfamily{phv}\fontseries{bc}\selectfont#1}%
\fi%
{\color{red}\sout{#2}}}

% \subst{Text to substitute}{Replacement}
% \subst[author]{Text to substitute}{Replacement}
\newcommand{\subst}[3][]{%
\if\relax\detokenize{#1}\relax%
\else\todo{\fontfamily{phv}\fontseries{bc}\selectfont#1}%
\fi%
{\color{red}\sout{#2}}{\color{teal}#3}}

